Scalable Learning of Non-Decomposable Objectives

Modern retrieval systems are often driven by an underlying machine learning model. The goal of such systems is to identify and possibly rank the few most relevant items for a given query or context. Thus, such systems are typically evaluated using a ranking-based performance metric such as the area under the precision-recall curve, the $F_\beta$ score, precision at fixed recall, etc. Obviously, it is desirable to train such systems to optimize the metric of interest. In practice, due to the scalability limitations of existing approaches for optimizing such objectives, large-scale retrieval systems are instead trained to maximize classification accuracy, in the hope that performance as measured via the true objective will also be favorable. In this work we present a unified framework that, using straightforward building block bounds, allows for highly scalable optimization of a wide range of ranking-based objectives. We demonstrate the advantage of our approach on several real-life retrieval problems that are significantly larger than those considered in the literature, while achieving substantial improvement in performance over the accuracy-objective baseline.

==> sandbox.tex <==
\section{Draft}
\subsection{Idea: Mini-Batch Gradient Steps}
\begin{enumerate}
\item Close form expression for the expectation of mini-batch for: $TP$,$P$, then $PR$,$RE$ and finally $AUC-PR$...
\item Convex upper bound on AUC see \cite{joachims2005support}
\item Onlien (batch) version of AUC-ROC.
\section{Expectation of batch $F_1$}
Start by considering  $\E[(\empirical{\precision},\empirical{\recall})]$ is it an unbiased estimate of $(\precision, \recall)$?
We start with understanding the precision and recall variables:
\begin{equation}\begin{split}
\Pr[\empirical{\precision}]  
  &= \sum_{k=1}^n \Pr[\empirical{\precision} \given \; |\empirical{\hat y}| = k ]\Pr[|\empirical{\hat y}| = k]
\end{split}\end{equation}

\begin{equation}\begin{split}
\empirical{\precision} &\sim \frac{1}{k} \sum_{k=1}^n  Bin(p\beta,n) \cdot Bin(p\beta + (1-p)(1-\alpha),n)
\end{split}\end{equation}

\begin{equation}\begin{split}
\Pr[\empirical{\recall}]  
  &= \sum_{k=1}^n \Pr[\empirical{\recall} \given \; |\empirical{y}| = k ]\Pr[|\empirical{y}| = k]
\end{split}\end{equation}

\begin{equation}\begin{split}
\empirical{\recall} &\sim \frac{1}{k} \sum_{k=1}^n  Bin(p\beta,n) \cdot Bin(p,n)
\end{split}\end{equation}


\subsection{Algorithm variants for $\aucpr$ ideas}
\begin{itemize}
\item For the $\recall@\precision$ task: rather than doing a binary search or a \emph{brute-force} approach to tune the class weights which achieves a given precision, we propose to dynamically shift the class-weight duding training. \enote{add code}
\item For the $\aucpr$ problem: while optimizing the setkeep $\th_1 \le \th_2 \ldots\th_k$ and so to compute the gradient we need only $\log(k)$ to search which $\th_i$ is non erroneous, then the gradient is something like $y_m \frac{i}{k} x_m$.
\item \todo{repeat with precision-recall-gain curves.}
\end{itemize}



